xFuzz: Machine Learning Guided Cross-Contract Fuzzing

Smart contract transactions are increasingly interleaved by cross-contract calls. While many tools have been developed to identify a common set of vulnerabilities, the cross-contract vulnerability is overlooked by existing tools. Cross-contract vulnerabilities are exploitable bugs that manifest in the presence of more than two interacting contracts. Existing methods are however limited to analyze a maximum of two contracts at the same time. Detecting cross-contract vulnerabilities is highly non-trivial. With multiple interacting contracts, the search space is much larger than that of a single contract. To address this problem, we present xFuzz, a machine learning guided smart contract fuzzing framework. The machine learning models are trained with novel features (e.g., word vectors and instructions) and are used to filter likely benign program paths. Comparing with existing static tools, machine learning model is proven to be more robust, avoiding directly adopting manually-defined rules in specific tools. We compare xFuzz with three state-of-the-art tools on 7,391 contracts. xFuzz detects 18 exploitable cross-contract vulnerabilities, of which 15 vulnerabilities are exposed for the first time. Furthermore, our approach is shown to be efficient in detecting non-cross-contract vulnerabilities as well -- using less than 20% time as that of other fuzzing tools, xFuzz detects twice as many vulnerabilities.

==> table/initialization.tex <==
\begin{table}[htb]
\caption{The number of files under ratios of mutation times on 54 contracts.}
\label{tbl:initialization}
\begin{tabular}{|c|c|c|c|}
\hline
$R_t \in (0,1]$ & $R_t = 1$ & $R_t \in (1,1000)$ & $R_t \in [1000,)$ \\ \hline
2               & 3         & 22                 & 27                \\ \hline
\end{tabular}
\small
\\
* Note that $R_t$ equals to $M_s/M_f$. $M_s$ denotes the mutation times of \sfuzz and $M_f$ denotes the mutation times after initial value changed. The higher $R_t$ is, the more efficiency the changed value brings.
\end{table}

==> table/parameter-weights.tex <==
\small
\begin{table}[h]
	\vspace{-3mm}
    \centering
    \caption{The weight of each type of paramenters.}
    \label{tbl:parameter weights}
    \begin{tabular}{|p{14mm}|p{10mm}|p{35mm}|}
 \hline
 Type Name & Weight & Description \\ 
 \hline
 address & 1 & address type \\
 \hline
 uint & 1.5 & including uint16, uint32, etc. \\
 \hline
 bytes & 2 & bytes of strings \\
 \hline
 bool & 1 & boolean type \\
 \hline
 array & 1.8 & array parameters \\
 \hline
\end{tabular}
\end{table}
\normalsize

==> table/rq2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{Detection precision and recall of \sfuzz and \textsc{sFuzzplus} when $t_l$ equals to 30s.}
\label{tbl:rq2-pr-rr}
\begin{tabular}{|c|cccc}
\hline
\multirow{2}{*}{} & \multicolumn{2}{c|}{Precision Rate} & \multicolumn{2}{c|}{Racall Rate} \\ \cline{2-5} 
 & \multicolumn{1}{l|}{sFuzz}  & \multicolumn{1}{l|}{sFuzzplus} & \multicolumn{1}{l|}{sFuzz}  & \multicolumn{1}{l|}{sFuzzplus} \\ \hline
Delegatecall & \multicolumn{1}{c|}{100\%} & \multicolumn{1}{c|}{100\%}  & \multicolumn{1}{c|}{57.6\%} & \multicolumn{1}{c|}{100\%}    \\ \hline
Reentrancy & \multicolumn{1}{c|}{100\%}  & \multicolumn{1}{c|}{100\%}  & \multicolumn{1}{c|}{33.9\%}  & \multicolumn{1}{c|}{99.2\%}  \\ \hline
\end{tabular}
\end{table}

==> table/sec5mutate.tex <==
\begin{table}[t]
\footnotesize
\centering

\caption{Mutation strategies of different priority scores.}
\label{tbl:sec5mutate}
% \begin{tabular}{cccccc}
% \toprule
% Priority Scores & \multicolumn{5}{c}{Mutation Strategies}      \\
% \midrule
% 1               & \multicolumn{5}{c}{bit flip}                 \\ 
% (1,10]          & bit flip & \multicolumn{4}{c}{bits flip}     \\ 
% (10, )          & bit flip & bits flip & reverse & concat & cut \\ 
% \bottomrule
% \end{tabular}
\begin{tabular}{cccccc} 
\toprule
Priority Scores & \multicolumn{5}{l}{Mutation Strategies} \\ 
\midrule
1 & bit flip &  &  &  &  \\
(1,10] & bit flip & bits flip &  &  &  \\
(10, ) & bit flip & bits flip & reverse & concat & cut \\
\bottomrule
\end{tabular}
\vspace{-0.4cm}
\end{table}

